ROS-related Robotic Systems Development with V-model-based Application of MeROS Metamodel

Systems built on the Robot Operating System (ROS) are increasingly easy to assemble, yet hard to govern and reliably coordinate. Beyond the sheer number of subsystems involved, the difficulty stems from their diversity and interaction depth. In this paper, we use a compact heterogeneous robotic system (HeROS), combining mobile and manipulation capabilities, as a demonstration vehicle under dynamically changing tasks. Notably, all its subsystems are powered by ROS. The use of compatible interfaces and other ROS integration capabilities simplifies the construction of such systems. However, this only addresses part of the complexity: the semantic coherence and structural traceability are even more important for precise coordination and call for deliberate engineering methods. The Model-Based Systems Engineering (MBSE) discipline, which emerged from the experience of complexity management in large-scale engineering domains, offers the methodological foundations needed. Despite their strengths in complementary aspects of robotics systems engineering, the lack of a unified approach to integrate ROS and MBSE hinders the full potential of these tools. Motivated by the anticipated impact of such a synergy in robotics practice, we propose a structured methodology based on MeROS - a SysML metamodel created specifically to put the ROS-based systems into the focus of the MBSE workflow. As its methodological backbone, we adapt the well-known V-model to this context, illustrating how complex robotic systems can be designed with traceability and validation capabilities embedded into their lifecycle using practices familiar to engineering teams.

==> MeROS_VModel_HeROS-RAS-Stereotypes.tex <==
% MeROS_VModel_HeROS-RAS-Preprint-Submission.tex

\RequirePackage{xparse}
\RequirePackage[T1]{fontenc}
\RequirePackage{xcolor}


\definecolor{StereotypeColor}{gray}{0.3}
\newcommand{\StereoFont}{\small\sffamily\mdseries}
\newcommand{\lguil}{\raisebox{0.1ex}{\scalebox{1.05}{\guillemotleft}}}
\newcommand{\rguil}{\raisebox{0.1ex}{\scalebox{1.05}{\guillemotright}}}

\newcommand{\stIsEmpty}[1]{
  \edef\stTmp{#1}
  \if\relax\detokenize{\stTmp}\relax
}

\ExplSyntaxOn
\NewDocumentCommand{\stereoCore}{ m m m }{%
  \group_begin:
  \tl_if_blank:nTF {#1}{\def\stPrefixProcessed{}}{\edef\stPrefixProcessed{#1-}}
  \textcolor{StereotypeColor}{\StereoFont{\textls[10]{\stPrefixProcessed\lguil#2\rguil#3}}}%
  \group_end:
}
\ExplSyntaxOff

\newcommand{\DeclareStereotype}[2]{%
  \expandafter\NewDocumentCommand\csname st#1\endcsname{ g D[]{} D[]{} }{%
    \stereoCore{##2}{#2}{##3}%
  }%
}

\DeclareStereotype{System}{Sy\-stem}
\DeclareStereotype{Node}{Node}
\DeclareStereotype{CLTool}{CL\-Tool}
\DeclareStereotype{Topic}{To\-pic}
\DeclareStereotype{Action}{Act\-ion}
\DeclareStereotype{Service}{Ser\-vice}
\DeclareStereotype{Parameter}{Para\-meter}
\DeclareStereotype{CommChannel}{Comm\-Chan\-nel}
\DeclareStereotype{ComponContain}{Com\-pon\-Con\-tain}
\DeclareStereotype{GpPackages}{Gp\-Packages}
\DeclareStereotype{Hardware}{Hardware}
\DeclareStereotype{LaunchFile}{Launch\-File}
\DeclareStereotype{MetaPackage}{Meta\-Package}
\DeclareStereotype{MicroNode}{Micro\-Node}
\DeclareStereotype{Namespace}{Name\-space}
\DeclareStereotype{Message}{Message}
\DeclareStereotype{Terminal}{Terminal}
\DeclareStereotype{Workspace}{Work\-space}
\DeclareStereotype{Package}{Pack\-age}
\DeclareStereotype{Repository}{Repo\-sitory}
\DeclareStereotype{RosCommCompon}{Ros\-Comm\-Com\-pon}
\DeclareStereotype{RosConnection}{Ros\-Conn\-ec\-tion}
\DeclareStereotype{RQtNode}{RQtNode}
\DeclareStereotype{RunSystemCompon}{Run\-System\-Compon}
\DeclareStereotype{SrcExeContain}{Src\-Exe\-Contain}
\DeclareStereotype{block}{block}
\DeclareStereotype{Requirement}{requirement}
\DeclareStereotype{Allocate}{allocate}

